Large-scale randomized-coordinate descent methods with non-separable linear constraints

We develop randomized (block) coordinate descent (CD) methods for linearly constrained convex optimization. Unlike most CD methods, we do not assume the constraints to be separable, but let them be coupled linearly. To our knowledge, ours is the first CD method that allows linear coupling constraints, without making the global iteration complexity have an exponential dependence on the number of constraints. We present algorithms and analysis for four key problem scenarios: (i) smooth; (ii) smooth + nonsmooth separable; (iii) asynchronous parallel; and (iv) stochastic. We illustrate empirical behavior of our algorithms by simulation experiments.

==> related.tex <==
%\begin{enumerate}
%\item \bibentry{liu2013asynchronousCD}
%\end{enumerate}

This paper consider convex problems of the form
\begin{align*}
  \min\quad f(x)\quad x \in C,
\end{align*}
where $C \subseteq \reals^n$ is a closed convex set.

They pay special attention to the unconstrained case $C=\reals^n$ and the fully separable case
\begin{align*}
  \min f(x)\quad x \in \nlprod_{i=1}^n C_i,
\end{align*}
where each $C_i$ is a compact interval.

\textbf{Highlights:}
\begin{itemize}
\setlength{\itemsep}{0pt}
\item Asychronous coordinate descent---multicore architecture.
\item Solution vector $x$ stored centrally, updated by each thread / core in an asynchronous fashion.
\item Update model similar to the Hogwild! method
\item Linear rate of convergence under ``essential strong convexity'' and $1/k$ for $C_L^1$ convex functions
\item Speedup controlled by $\tau$ and its play-off against $n$
\item Method is of the ``coordinate gradient descent'' type
\item Convergence analysis involves $L_{res}$ and $L_{\max}$, where $\norm{\nabla f(x) - \nabla f(x+ t e_i)} \le L_{res}|t|$ for $1 \le i \le n$ and $x, x+te_i \in C$. The constant $L_{res}$ is a bound on $\pnorm{\nabla^2 f}{\infty,2}$ (max column norm)
\item This shows that the tradeoffs are going to be between how strong the diagonals are, since $L_{\max}=\max_{1\le i \le n} L_i$
\item Multiple processors have access to a shared data vector $x$. Each processor is assumed to be able to compute a randomly chosen element of the gradient vector $\nabla f(x)$---this choice makes it impractical for a distributed setting, but reasonable for a shared memory multiprocessor (due to randomization, memory access is nonlinear and contentious so also not that suitable for GPUs)
\item Stepsizes depend on $L_{\max}$ which may be too pessimistic
\item The delay bound $\tau$ is traded-off in terms of the $L_{res}/L_{\max}$ ratio and $n$. Notice that the linear rate has a contraction coefficient $(1-1/(nL))$ so that as dimensionality grows, the method becomes essentially sublinear.
\item Some experiments on simple setups show almost linear speedups---this cannot be sustainable in general
\end{itemize}

\textbf{NOTE:}
\begin{itemize}
\item  We should also permit ``essential strong convexity'' (or at least comment on it)
\end{itemize}

\section{List of work to potentially summarize}

\subsection{Proximal methods}
\begin{enumerate}
\item FBS
\item Nesterov's accelerated prox-gradient (Beck and Teboulle 2009, Nesterov 2007)
\item Prox operator can be quite demanding or require substantial effort to implement efficiently (e.g, prox-TV, Mairal et al Tree method or Network Flow methods)
\end{enumerate}

\subsection{Coordinate descent}
\begin{enumerate}
\item Cyclic coordinate descent -- Tseng (a few papers, cite some of these, including later work by Tseng and Yun)
\item Classical paper on local linear convergence of CD (Tseng and Luo 1992)
\item Global linear under additional assumptions -- Wang and Lin 2013
\item Global rates for BCD more recently studied by Beck and Tetruashvili (2013), including 2-block case
\item Newton CD by Hsieh-et al maybe?
\item Improved local convergence by Wright 2012
\item Nesterov (2012) first to prove randomized CD rates -- linear and sublinear
\item Extensions of that (with slightly modified analysis) to composite functions by Richtarik and Takac (2011); see also Lu and Xiao
\item Everybody uses actually CGD (not pure CD)
\item Stochastic DCA of Shalev-Shwartz et al
\item Goldfarb and Ma (2012) based on multiple splitting
\item Luo et al. (2013) --- multiblock Gauss-Seidel style ADMM
\item Other parallel ADMM style approaches in general
\item \emph{Synchronous parallel:} Ferris \& Mangasarian's (1994); RT (2012) for convex composite problems---all processors update randomly selected coordinate blocks \emph{concurrently and synchronously}. Whether there is speedup or not depends on sparsity / overlap pattern determined by the input data matrix. Strategies for greedily selecting blocks of coordinates have also been studied---
\item \emph{Asynchronous parallel:} Bertsekas and Tsitsiklis (1989) allow \emph{inconsistent} reads---linear convergence via fixed-point analysis is established provided all ``ages'' are bounded and the Hessian is diagonally dominant. Liu et al prove linear convergence without DD but do not allow inconsistent reads.
\end{enumerate}

\subsection{Subgradient style}
\begin{enumerate}
\item Ofer Dekel -- for parallel minibatch
\item Richtarik and Takac --- improved minibatching based on spectral properties of input data
\item Duchi, Agarwal, Wainright --- dual averaging for distributed
\item Agarwal, Duchi -- distributed, delayed stoch gradients
\item Cotter, Shamir, Srebro, Sridharan --- minibatch SG with Nesterov acceleration
\item Other parallel stochastic gradient methods (mostly the minibatch idea)
\item Subgradient methods with variance reduction: SAG, SVRG, prox-SVRG
\item Hogwild! -- lock free, asynchronous, multicore SGD method --- also assumes consistent reading of the variable $x$
\item Avron et al---asynchronous linear rate solver for $Ax=b$ (with randomization)
\end{enumerate}

\subsection{FW methods}

\begin{enumerate}
\item Cite the 1956 FW paper
\item FW work of Hazan 2008, interest generated by Clarkson's paper (2010) (where apparently the curvature quantity was introduced);
\item Bach---duality between subgradient and conditional gradient
\item Conditional gradient method (Bertsekas' textbook), and more recently Yaoliang's GCG which allows a regularizer
\item Other relevant FW papers: Freund and Grigas (New analysis and result for conditional gradinet), Jaggi and Sulovsky, 2010 (A simple algorithm for nuclear norm regularized problems). Particularly nice overview (including definition of the simpler duality gap) in Jaggi, 2013 (Revisiting Frank-Wolfe: projection-free sparse convex optimization); Cite also the NIPS 2013 workshop on FW methods. See also the additional related work in the GCG paper.
\item BCFW -- they propose a randomized BC version of FW -- the iteration arithmetic cost as well as complexity are similar to that of stochastic gradient descent. However, BCFW can be advantageous because: (a) in some cases, the optimal step size can be computed in closed-form, which saves the pain of unavoidable stepsize tuning; (b) duality gap guarantee to give confidence about constraints (c) convergence rate analysis extends to handle inexact linear minimization oracles; (d) linear subproblems are typically easier to solve than projection.

BCFW reduces \textbf{but does not eliminate} the need to go through all the training data?

\item FW methods also shine when working with matrices, where the cost of a projection starts dominating; best example is the trace-norm constrained problems that solve relaxations of low-rank matrix approximation problems: here solving a linear problem over the trace-norm ball constraint requires just the maximum singular vectors (which can be computed quite rapidly using PROPACK, or SLEPSc in parallel); the projection problems require the full SVD, which completely destroys practicality for large matrices.
\end{enumerate}

\subsection{Architecturally closest methods}
\begin{enumerate}
\item AsyncCD method of Liu et al
\item Hogwild! is related, as are the slew of parallel coordinate descent methods of Richtarik and Takac
\end{enumerate}

\subsection{Comments on the parallelism}
\begin{enumerate}
\item Asynchronous parallel is the structure; some discussion of pure distributed case provided toward end of paper.
\item Careful analysis that shows ``data dependent'' speedups due to parallelism (a discussion / commentary about $\tau$ is needed, including how similar considerations appear in the CD work of Richtarik, in the theory of mini-batched Stochastic gradient methods, in the AsyncCD method, also in SDCA)---the point being that without careful exploitation of data dependent structure the analysis typically yields no theoretical speedup due to $\tau > 1$ (see discussion in \S\ref{sec:}). However,
\end{enumerate}

\subsection{Related work for Applications}
\begin{enumerate}
\item Structural SVM
\item
\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "coordNips"
%%% End:

